SigNet: Convolutional Siamese Network for Writer Independent Offline Signature Verification

Offline signature verification is one of the most challenging tasks in biometrics and document forensics. Unlike other verification problems, it needs to model minute but critical details between genuine and forged signatures, because a skilled falsification might often resembles the real signature with small deformation. This verification task is even harder in writer independent scenarios which is undeniably fiscal for realistic cases. In this paper, we model an offline writer independent signature verification task with a convolutional Siamese network. Siamese networks are twin networks with shared weights, which can be trained to learn a feature space where similar observations are placed in proximity. This is achieved by exposing the network to a pair of similar and dissimilar observations and minimizing the Euclidean distance between similar pairs while simultaneously maximizing it between dissimilar pairs. Experiments conducted on cross-domain datasets emphasize the capability of our network to model forgery in different languages (scripts) and handwriting styles. Moreover, our designed Siamese network, named SigNet, exceeds the state-of-the-art results on most of the benchmark signature datasets, which paves the way for further research in this direction.

==> extras.tex <==

\thispagestyle{empty}
                                                             
\begin{table*}[!th]

\begin{minipage}{.9\textwidth}
\baselineskip12pt
\ifpreprint
  \vspace*{1pc}
\else
  \vspace*{-6pc}
\fi

\noindent {\LARGE\itshape Pattern Recognition Letters}
\vskip6pt

\noindent {\Large\bfseries Authorship Confirmation}

\vskip1pc


{\bf Please save a copy of this file, complete and upload as the 
``Confirmation of Authorship'' file.}

\vskip1pc

As corresponding author 
I, \underline{\hphantom{\hspace*{7cm}}}, 
hereby confirm on behalf of all authors that:

\vskip1pc

\begin{enumerate}
\itemsep=3pt
\item This manuscript, or a large part of it, \underline {has not been
published,  was not, and is not being submitted to} any other journal. 

\item If \underline {presented} at or \underline {submitted} to or
\underline  {published }at a conference(s), the conference(s) is (are)
identified and  substantial \underline {justification for
re-publication} is presented  below. A \underline {copy of
conference paper(s) }is(are) uploaded with the  manuscript.

\item If the manuscript appears as a preprint anywhere on the web, e.g.
arXiv,  etc., it is identified below. The \underline {preprint should
include a  statement that the paper is under consideration at Pattern
Recognition  Letters}.

\item All text and graphics, except for those marked with sources, are
\underline  {original works} of the authors, and all necessary
permissions for  publication were secured prior to submission of the
manuscript.

\item All authors each made a significant contribution to the research
reported  and have \underline {read} and \underline {approved} the
submitted  manuscript. 
\end{enumerate}

Signature\underline{\hphantom{\hspace*{7cm}}} Date\underline{\hphantom{\hspace*{4cm}}} 
\vskip1pc

\rule{\textwidth}{2pt}
\vskip1pc

{\bf List any pre-prints:}
\vskip5pc


\rule{\textwidth}{2pt}
\vskip1pc

{\bf Relevant Conference publication(s) (submitted, accepted, or
published):}
\vskip5pc


{\bf Justification for re-publication:}

\end{minipage}
\end{table*}

\clearpage
\thispagestyle{empty}
\ifpreprint
  \vspace*{-1pc}
\fi

\begin{table*}[!th]
\ifpreprint\else\vspace*{-5pc}\fi

\section*{Graphical Abstract (Optional)}
To create your abstract, please type over the instructions in the template box below. Fonts or abstract dimensions should not be changed or altered. 

\vskip1pc
\fbox{
\begin{tabular}{p{.96\textwidth}}
\bf SigNet: Convolutional Siamese Network for Writer Independent Offline Signature Verification \\
Sounak \snm{Dey}, Anjan \snm{Dutta}, Suman K. \snm{Ghosh}, J. Ignacio \snm{Toledo}, Josep \snm{Llad\'{o}s}, Umapada \snm{Pal} \\[1pc]
\begin{center}
\includegraphics[width=.8\textwidth]{arch_signet}
\end{center}
\end{tabular}
}

\end{table*}

\clearpage
\thispagestyle{empty}

\ifpreprint
  \vspace*{-1pc}
\else
%  \vspace*{-6pc}
\fi

\begin{table*}[!t]
\ifpreprint\else\vspace*{-15pc}\fi

\section*{Research Highlights (Required)}

To create your highlights, please type the highlights against each
\verb+\item+ command. 

\vskip1pc

\fboxsep=6pt
\fbox{
\begin{minipage}{.95\textwidth}
It should be short collection of bullet points that convey the core findings of the article. It should  include 3 to 5 bullet points (maximum 85 characters, including spaces, per bullet point.)  
\vskip1pc
\begin{itemize}

\item A convolution Siamese network is proposed for Offline signature verification.

\item To our knowledge Siamese network has not been used for offline signature verification.
 
\item The proposed model shows better results than the state of the art results.

 % \item 

\end{itemize}
\vskip1pc
\end{minipage}
}

\end{table*}

\clearpage


\ifpreprint
  \setcounter{page}{1}
\else
  \setcounter{page}{1}
\fi

